Automatic Horizontal Fusion for GPU Kernels

We present automatic horizontal fusion, a novel optimization technique that complements the standard kernel fusion techniques for GPU programs. Unlike the standard fusion, whose goal is to eliminate intermediate data round trips, our horizontal fusion technique aims to increase the thread-level parallelism to hide instruction latencies. We also present HFuse, a new source to source CUDA compiler that implements automatic horizontal fusion. Our experimental results show that horizontal fusion can speed up the running time by 2.5%-60.8%. Our results reveal that the horizontal fusion is especially beneficial for fusing kernels with instructions that require different kinds of GPU resources (e.g., a memory-intensive kernel and a compute-intensive kernel).

==> figs/decoration.tex <==
\SetEndCharOfAlgoLine{}
\Input{A list of statement $S$, the lower bound $a$ and
upper bound $b$ of the thread index assigned to the kernel.}
\Output{A list of pairs, where the first element is a basic synchronization part and the second is the corresponding barrier statement.}
\underline{function} $\mathrm{TranslateParts}(S, a, b):$\\

$S'\leftarrow \mathrm{Instrument}(S, a, b)$

$B\leftarrow\emptyset$

$P\leftarrow\emptyset$

\For {$s\in S'$} {

  \If {$\mathrm{HasBarrier}(s)$} {
    $B\leftarrow B\circ\langle P, s\rangle$

    $P\leftarrow\emptyset$
  }
  \Else {
    Append $s$ to $P$
  }
}

$B\leftarrow B\circ\langle P, \text{Nil}\rangle$

\Return $B$

\underline{function} $\mathrm{Instrument}(S, a, b):$\\

$l\leftarrow \text{a new fresh label}$

$S'\leftarrow \emptyset$

Append ``\text{if (threadIdx.x < $a$ || threadIdx.x >= $b$) goto $l$}'' to $S'$

\For {$s\in S$} {

  \If {$s$ is an if or loop statement and $S'$ is the body statement list} {
    $S''\in \mathrm{Instrument}(S', a, b)$

    Replace the body statement list in $s$ with $S''$
  }

  \If {$\mathrm{HasBarrier}(s)$} {
    Mark $s$ with the label $l$ and append $s$ to $S'$

    $l\leftarrow \text{a new fresh label}$

    Append ``\text{if (threadIdx.x < $a$ || threadIdx.y >= $b$) goto $l$}" to $S'$
  }
  \Else {
    Append $s$ to $S'$
  }
}

Mark the end of $S'$ with the label $l$

\Return $S'$


==> files/__latexindent_temp.tex <==
  SIA & 30.2 & 90.47 & 23.40 & 22.92 & 1.31 & 0.49 & 9.88 &  \\
   \hline
  Ethash+Blake & 52.9 & 64.62 & 39.43 & 9.97 & 22.86 & 0.31 & 5.18 & \multirow{2}{*}{4.86} \\
Ethash+Blake (Spill) & 47.7 & 71.65 & 42.80 & 8.19 & 17.38 & 0.41 & 6.59 &  \\
   \hline
  Ethash+SIA & 54.0 & 67.62 & 36.47 & 9.54 & 26.33 & 0.31 & 5.29 & \multirow{2}{*}{4.30} \\
Ethash+SIA (Spill) & 48.3 & 71.00 & 42.93 & 7.83 & 17.43 & 0.40 & 6.56 &  \\
   \hline
  Ethash+SHA256 & 67.2 & 32.99 & 60.51 & 6.78 & 13.35 & 0.17 & 2.00 & \multirow{2}{*}{2.49} \\
Ethash+SHA256 (Spill) & 55.1 & 41.90 & 33.67 & 6.55 & 43.13 & 0.41 & 3.06 &  \\
   \hline
  Blake+SIA & 67.3 & 85.23 & 43.48 & 15.40 & 1.32 & 0.49 & 8.73 & \multirow{2}{*}{10.57} \\
Blake+SIA (Spill) & 69.8 & 85.29 & 46.39 & 12.81 & 1.24 & 0.49 & 8.78 &  \\
   \hline
  Blake+SHA256 & 121.0 & 38.55 & 72.84 & 6.00 & 0.69 & 0.21 & 2.55 & \multirow{2}{*}{8.62} \\
Blake+SHA256 (Spill) & 62.0 & 75.44 & 53.12 & 7.30 & 1.52 & 0.43 & 7.20 &  \\
   \hline
  SIA+SHA256 & 116.5 & 38.82 & 72.22 & 6.05 & 1.14 & 0.21 & 2.55 & \multirow{2}{*}{7.89} \\
SIA+SHA256 (Spill) & 63.0 & 75.82 & 52.79 & 7.15 & 1.72 & 0.44 & 7.17 &  \\
   \hline
